A Causal Ordering Prior for Unsupervised Representation Learning

Unsupervised representation learning with variational inference relies heavily on independence assumptions over latent variables. Causal representation learning (CRL), however, argues that factors of variation in a dataset are, in fact, causally related. Allowing latent variables to be correlated, as a consequence of causal relationships, is more realistic and generalisable. So far, provably identifiable methods rely on: auxiliary information, weak labels, and interventional or even counterfactual data. Inspired by causal discovery with functional causal models, we propose a fully unsupervised representation learning method that considers a data generation process with a latent additive noise model (ANM). We encourage the latent space to follow a causal ordering via loss function based on the Hessian of the latent distribution.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}


\end{enumerate}

==> prelimnaries.tex <==
% \begin{figure}[!ht]
%     \centering
%     \begin{subfigure}{.20\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node[obs] (x) {$\mathbf{x}$};
%             \node[obs, left=of x] (pa) {$\mathbf{pa}$};
%             \node[latent, above right=0.55cm of pa] (z) {$\mathbf{z}$};

%             \edge{pa}{x}
%             \edge{z}{pa}
%             \edge{z}{x}
            
%         \end{tikzpicture}
%         \caption{Conditional}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.20\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node[obs] (x) {$\mathbf{x}$};
%             \node[obs, left=of x] (pa) {$\mathbf{pa}$};
%             \node[latent, above right=0.55cm of pa, ] (z) {$\mathbf{z}$};

%             \edge{pa}{x}
%             \edge{pa}{z}
%             \edge{z}{x}
            
%         \end{tikzpicture}
%         \caption{Mediator}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.20\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node[obs] (x) {$\mathbf{x}$};
%             \node[obs, left=of x] (pa) {$\mathbf{pa}$};
%             \node[latent, above right=0.55cm of pa, ] (z) {$\mathbf{z}$};

%             \edge{pa}{x}
%             \edge{z}{x}
            
%         \end{tikzpicture}
%         \caption{Disjoint}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.20\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node[obs] (x) {$\mathbf{x}$};
%             \node[latent, left=of x] (z) {$\mathbf{z}$};
%             \node[latent, above right=0.55cm of pa, ] (epsx) {$\mathbf{\epsilon}_x$};

%             \edge{z}{x}
%             \edge{epsx}{x}
%         \end{tikzpicture}
%         \caption{Implicit}
%     \end{subfigure}
%     \caption{In our proposed method $\mathbf{pa} = \mathbf{z}$.}
% \end{figure}



% \begin{definition}(Mean Conditional Independence, MCI)
% Given topologically ordered set of random variables $\rmX = \{\rmX_0, \dots, \rmX_d\}$, MCI is defined as:
% \begin{equation}
%     \textsc{MCI}(\rmX) = \sum^{d-2}_i \frac{1}{3}\textsc{HSCIC}(\rmX_i, \rmX_{i+2} \mid \rmX_{i+1}) + \frac{2}{3}\textsc{HSCIC}(\rmX_i, \rmX_{i+1} \mid \rmX_{i+2})
%     \label{eqn:mci}
% \end{equation}
% where $\textsc{HSCIC}$ is \emph{Hilbert-Schmidt Conditional Independence Criterion} as defined in \cite{measure.theoretic.Approach}. 
% \end{definition}
% \begin{remark}

%  \begin{figure}[!ht]
%     \centering
%     \begin{subfigure}{.18\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node[obs, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x1) {$\mathbf{\rmX}_i$};
%             \node[obs, left=0.5cm of x, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x2) {$\mathbf{\rmX}_{i+1}$};
%             \node[obs, above=0.35cm of x2, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x3) {$\mathbf{\rmX}_{i+2}$};

%             \edge{x2}{x1}
%             \edge{x3}{x2}
%         \end{tikzpicture}
%         \caption{}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.18\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node[obs, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x1) {$\mathbf{\rmX}_i$};
%             \node[obs, left=0.5cm of x, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x2) {$\mathbf{\rmX}_{i+1}$};
%             \node[obs, above=0.35cm of x2, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x3) {$\mathbf{\rmX}_{i+2}$};

%         \end{tikzpicture}
%         \caption{}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.18\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node[obs, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x1) {$\mathbf{\rmX}_i$};
%             \node[obs, left=0.5cm of x, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x2) {$\mathbf{\rmX}_{i+1}$};
%             \node[obs, above=0.35cm of x2, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x3) {$\mathbf{\rmX}_{i+2}$};

%             \edge{x3}{x1}
%             \edge{x3}{x2}
%         \end{tikzpicture}
%         \caption{}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.18\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node[obs, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x1) {$\mathbf{\rmX}_i$};
%             \node[obs, left=0.5cm of x, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x2) {$\mathbf{\rmX}_{i+1}$};
%             \node[obs, above=0.35cm of x2, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x3) {$\mathbf{\rmX}_{i+2}$};

%             \edge{x3}{x2}
%         \end{tikzpicture}
%         \caption{}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.18\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node[obs, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x1) {$\mathbf{\rmX}_i$};
%             \node[obs, left=0.5cm of x, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x2) {$\mathbf{\rmX}_{i+1}$};
%             \node[obs, above=0.35cm of x2, minimum size=20pt, font=\fontsize{3}{3}\selectfont] (x3) {$\mathbf{\rmX}_{i+2}$};

%             \edge{x3}{x1}
%         \end{tikzpicture}
%         \caption{}
%     \end{subfigure}
%     \caption{In case of topological ordered variables, the causal graph can be factorized as one of the above, decomposition (a) and (b) satisfy the conditional independence $\rmX_{i} \perp \rmX_{i+2} || \rmX_{i+1}$ while the decomposition (b), (c), (d), and (e) satisfy $\rmX_{i} \perp \rmX_{i+1} || \rmX_{i+2}$. Due to this reason factor (1/3) and (2/3) are assigned to conditions respectively. Remaining factorizations like cliques cannot be measured by conditional independence of the considered form.} 
% \end{figure}   
% \end{remark}
